Best of Both Worlds: Enforcing Detailed Balance in Machine Learning Models of Transition Rates

The slow microstructural evolution of materials often plays a key role in determining material properties. When the unit steps of the evolution process are slow, direct simulation approaches such as molecular dynamics become prohibitive and Kinetic Monte-Carlo (kMC) algorithms, where the state-to-state evolution of the system is represented in terms of a continuous-time Markov chain, are instead frequently relied upon to efficiently predict long-time evolution. The accuracy of kMC simulations however relies on the complete and accurate knowledge of reaction pathways and corresponding kinetics. This requirement becomes extremely stringent in complex systems such as concentrated alloys where the astronomical number of local atomic configurations makes the a priori tabulation of all possible transitions impractical. Machine learning models of transition kinetics have been used to mitigate this problem by enabling the efficient on-the-fly prediction of kinetic parameters. In this study, we show how physics-informed ML architectures can exactly enforce the detailed balance condition, by construction. Using the diffusion of a vacancy in a concentrated alloy as an example, we show that such ML architectures also exhibit superior performance in terms of prediction accuracy, demonstrating that the imposition of physical constraints can facilitate the accurate learning of barriers at no increase in computational cost.

==> Introduction.tex <==
\section*{Introduction}
Many key processes controlling defect evolution in materials are associated with the crossing of large energy barriers, and hence occur on very long timescales. This often makes the simulation of microstructure evolution, which is critical to the prediction of many material properties, prohibitively expensive using direct methods such as molecular dynamics ~\cite{uberuaga2020computational}. 
A common modeling approach that dramatically reduces the computational cost of long timescale simulations is the so-called kinetic Monte Carlo (kMC) approach~\cite{voter2007introduction}, 
where the evolution of the material is approximated as a continuous time Markov chain expressed on a discrete state space that corresponds to the different long-lived conformations of the system. In addition to the set of possible states, a kMC model also requires the specification of the state-to-state transition rates along all possible reaction pathways. This representation makes it possible to numerically sample long state-to-state trajectories extremely efficiently, thereby enabling long-timescale simulations. The fidelity of kMC simulations with respect to direct molecular dynamics however relies on the completeness of the set of states and transitions included in the model, on the numerical accuracy of the estimated transition rates between states, and on the state-to-state transitions being sufficiently rare~\cite{di2016jump,aristoff2023arbitrarily}. 

In traditional kMC simulations, transition rates are typically expressed in terms of Arrhenius expressions where the prefactors and barriers corresponding to different transition pathways are tabulated {\em a priori}~\cite{voter2007introduction}. In more modern incarnations, \cite{henkelman2001long,beland2011kinetic} transition catalogues are constructed on-the-fly using direct saddle search methods. These approaches are especially powerful for "simple" materials (e.g., elemental solids); however, the combinatorial explosion in the number of required energy barriers for chemically (i.e., concentrated alloys) or topologically (i.e., glassy) complex materials can significantly increase their computational cost. In the following, we concentrate on the problem of simulating the diffusion of defects in chemically complex systems, where the number of topologically-distinct transition pathways is  limited, but the number of possible "decorations" of the initial and final states by different chemical environments is astronomical. As each event requires its own transition rate, {\em a priori} tabulation  is often not feasible, while on-the-fly computation using direct saddle search methods incurs a significant computational cost. In order to address this limitation, machine learning (ML) models have been introduced as valuable alternatives to direct computation, which have the potential to restore high simulation rates and long simulation timescales, while preserving high fidelity.
A number of ML models have been developed to model defect migration energetics in alloys, typically requiring on the order of $10^3 -10^4$ explicit barrier calculations for training \cite{manzoor2021machine, fan2022predicting, xu2022revealing, huang2023high}, which in concentrated alloys can be a very small fraction of the total chemical space, leading to potentially considerable computational speedups.

For example, Pascuet~\etal~\cite{pascuet2011stability} were one of the first to predict the migration barriers of Cu vacancy clusters $V_n$ for 1$\leq$n$\leq$6 in Fe using Artificial Neural Network (ANN) models to gain insight into the stability and mobility of mixed copper–vacancy clusters, which play a key role in copper precipitation in iron alloys under irradiation. Castin~\etal also used ANNs  to predict vacancy migration energies as functions of the local atomic environment in Fe-based alloys~\cite{castin2010calculation,castin2018advanced}. Datasets of migration barriers for nearest-neighbour jumps on the Cu surfaces were calculated with the nudged elastic band (NEB) method and the tethering force approach of Kimari~\etal~\cite{kimari2020data} and used to train ANN models to predict the migration barriers for arbitrary nearest-neighbour Cu jumps. 
Fan \etal developed a convolutional neural network (CNN)—based model to predict the path-dependent vacancy migration energy barrier spectra in the TaNbMo multi-principal element alloy, using local chemical features surrounding each vacancy extracted via spatial density maps (SDMs)~\cite{fan2021predicting}.  Their framework can be applied to predict barriers in both crystalline materials~\cite{fan2021predicting} and amorphous materials~\cite{fan2022predicting2}. Lapointe \etal~\cite{lapointe2022machine} implemented a nonlinear surrogate model approach to learn and predict the kinetic transition rates during defect migration in $\alpha$-iron and amorphous Si systems. They show that it is possible to predict the formation entropy of defects and the logarithm of the prefactor of their activated events with only $O(N)$ numerical computations, which avoids the time-consuming evaluation of the system’s dynamical matrix $(O(N^2))$ and its spectrum $(O(N^3))$.
In their study of vacancy-mediated sluggish diffusion in concentrated Ni-Fe model alloys, Huang \etal~\cite{huang2023machine} used about 32,000 pre-calculated NEB~\cite{jonsson1998nudged, henkelman2000climbing} barriers to train an ANN-based machine learning model to predict the vacancy migration barriers for arbitrary local atomic environments, including both random solution configurations and alloys with short-range ordering.   

While these efforts have demonstrated the power of ML-guided kMC models to simulate defect evolution in complex alloys, none have considered whether the resulting kMC models obey key physical constraints. In particular, one important physical constraint is the so-called detailed balance condition (DBC). The DBC is a cornerstone of Monte Carlo methods since it provides a simple guarantee that an algorithm will sample from a well-defined stationary distribution in the long-time limit. While the DBC is a sufficient condition for the existence of a stationary distribution, it is not strictly necessary, as weaker conditions such as global balance can provide the same guarantees \cite{bernard2009event}. However, the DBC is typically much simpler to impose as it can naturally be enforced when transition rates are derived from Transition State Theory (TST).
 
In this paper, we investigate physics-informed generalizations of this type of ML approach, focusing on the imposition of the DBC. In the following, we mathematically demonstrate that the DBC-preserving structure of TST can be used to design ML architectures that are also guaranteed to exactly obey the DBC {\em by construction}. Using vacancy diffusion in concentrated alloys as an example,
we investigate the performance of different ML variants that attempt to impose the DBC using different non-strict strategies in order to identify possible trade-offs between accuracy of the prediction of individual rates and the extent to which the DBC is enforced. We find that architectures that strictly impose the DBC by construction in fact exhibit lower errors than their inexact counterparts, suggesting that the introduction of physically-motivated constraints in fact assists the learning process, providing higher-quality models that obey physical constraints without increasing the computational cost.

